Order Statistics Approaches to Unobserved Heterogeneity in Auctions

We establish nonparametric identification of auction models with continuous and nonseparable unobserved heterogeneity using three consecutive order statistics of bids. We then propose sieve maximum likelihood estimators for the joint distribution of unobserved heterogeneity and the private value, as well as their conditional and marginal distributions. Lastly, we apply our methodology to a novel dataset from judicial auctions in China. Our estimates suggest substantial gains from accounting for unobserved heterogeneity when setting reserve prices. We propose a simple scheme that achieves nearly optimal revenue by using the appraisal value as the reserve price.

==> dump.tex <==
%{\color{red} Yao: We haven't shown why $\{\frac{f}{f}:x^*\in \mathcal{X}^*\}$ is a close set and hence the spectrum is. @Peijun??? the proof seems to ``assume'' $\{\frac{f}{f}:x^*\in \mathcal{X}^*\}$ is an interval?  btw, the next sentence, is it "The spectrum $\sigma$ OF $JJ^{-1}$ is?"}

%{\color{red} Ruli: Is $J_{y_1} J_{y_2}^{-1}$ is bounded? If $J_{y_2}$ is bounded, its inverse is also bounded, right? HS used the bounded assumption in the $y$ and $x$ relationship to say that the largest element of the spectrum is bounded so the operator is indeed bounded in the sense required by Dunford and Schwarz's result. Any idea what does this mean? Our eigenvalues is the ratio while that in HS is just $f(y|\tau)$, but I guess the bounded condition still applies in our context, right? It seems that the spectrum always contains all eigenvalues but not limited to them, meaning that spectrum might be larger than the set of the eigenvalues. Do we get the spectrum from the eigenfunction decomposition instead of eigenvalues? so we need to show that the spectrum is the same as the set of all eigenvalues? So the referee is asking about why the spectrum the same as the set of eigenvalues? Did Hu have the same issues? How do they solve it then?}

%The spectrum $\sigma$ is $J_{y_1}J_{y_2}^{-1}$ is  actually the range of $\left\{\frac{f^{X|\Xst}(y_1 | \xst)}{f^{X|\Xst}(y_2 | \xst)}: \xst \in \XXst\right\}$, which is denoted by $[\lambda_1(y_1, y_2), \lambda_2(y_1, y_2)]$. 

%Some comments on unbounded operators and inverse operators.

%In our setting, $L_{X_{r-2:r-2}|\Xst}$ is an integral operator. We first claim that its range is not an closed subset in the image space. To verify this statement, we use the following property:  a bounded linear map $T$
%between Banach spaces is injective with closed range if and only if it is bounded below, i.e. $\|Tx\| \geq c\|x\|$ for any $x$ in the domain for some positive constant $c$. However, it is straightforward to show that $L_{X_{r-2:r-2}|\Xst}$ is a compact operator. Hence it cannot be bounded from below. Therefore, its range is not a closed subset in the image space, and thus, the inverse of $L_{X_{r-2:r-2}|\Xst}$ can be defined on range $L_{X_{r-2:r-2}|\Xst} \oplus \text{range} L_{X_{r-2:r-2}|\Xst}^{\perp}$, which is a dense subset of the image space of $L_{X_{r-2:r-2}|\Xst}$. {\color{red}Yao: Why do we need to define S here? } Let $\mathcal S = L_{X_{r-2:r-2}|\Xst} \oplus \text{range} L_{X_{r-2:r-2}|\Xst}^{\perp}$. {\color{red}Yao: Why set to zero here? Does it make a point? RX: is setting to zero to supplement the definition of the inverse?} 
%{\color {blue} Peijun: you do not have to set it to be zero, but this is a commonly used way to make the inverse defined over a dense subset to $\mathcal S$. We do not have to define $\mathcal S$. What I wrote is to give a clear explanation to Prof Hu. about my understanding towards this problem.}
%We set the inverse equal to zero on the orthogonal complement of $\text{range} L_{X_{r-2:r-2}|\Xst}$. However, I have no idea how to extend the inverse operator to the whole image space of $L_{X_{r-2:r-2}|\Xst}$. 

%{\color{red}[RX: What we discuss above is that the inverse operator can be bounded in a dense subset of the image space of the original operator, right? And together with the fact that the  spectrum of $L_{X_{r-2:r-2}|\Xst}\mathcal{D}_{y_1, y_2 }L_{X_{r-2:r-2}|\Xst}^{-1}$ is a compact set that does not contain 0, we then can claim that the operator $J_{y_1} J_{y_2}^{-1}$ is bound in a dense subset? Do we have any reference on this or it should be something from a textbook? Therefore we can claim to have unique decomposition for $J_{y_1} J_{y_2}^{-1}$ by following the theorem in the Dunford book, Right?]}

%{\color{blue}{I do not know whether the inverse operator defined over this dense subset is bounded or not. Additionally, I do not think it is important to verify it is bounded. We only need to show the sandwich operator is bounded. I believe that is sufficient. The operator is bounded because the operator is positive  and its spectrum is a bounded closed interval. }

%Next we will show that the spectrum of $L_{X_{r-2:r-2}|\Xst}\mathcal{D}_{y_1, y_2 }L_{X_{r-2:r-2}|\Xst}^{-1}$ is a compact set that does not contain 0.
%Denote the range of $\left\{\frac{f^{X|\Xst}(y_1 | \xst)}{f^{X|\Xst}(y_2 | \xst)}: \xst \in \XXst\right\}$ as $\mathcal{I} = [\lambda_1(y_1, y_2), \lambda_2(y_1, y_2)]$. Define $\mathcal{D}_{y_1, y_2}$ as an operator from 
%	$\mL^2(\XXst)$ to $\mL^2(\XXst)$ such that 
	$$
%	(\mathcal{D}_{y_1, y_2} g)(\tau) = \frac{f^{X|\Xst}(y_1 | \xst)}{f^{X|\Xst}(y_2 | \xst)} g(\tau)
	$$
%	for any $g \in \mL^2(\XXst)$. We now show that the spectrum of $\mathcal{D}_{y_1, y_2 }$, denoted by $\sigma_{\mathcal{D}}$, is $\mathcal{I}$. 


%Step 1: Note that lemma 1 establishes that the inverse operator $L_{X_{r-2:r-2}|\Xst}$ is defined over a dense subset of $\mathcal L^2(\mathcal A_l)$. 
%I think the reason why it cannot defined over the whole space is not important. If you are interested, you can refer to the following argument. In our setting, $L_{X_{r-2:r-2}|\Xst}$ is an integral operator. We first claim that its range is not an closed subset in the image space. To verify this statement, we use the following property:  a bounded linear map $T$between Banach spaces is injective with closed range if and only if it is bounded below, i.e. $\|Tx\| \geq c\|x\|$ for any $x$ in the domain for some positive constant $c$. However, it is straightforward to show that $L_{X_{r-2:r-2}|\Xst}$ is a compact operator. Hence it cannot be bounded from below. Therefore, its range is not a closed subset in the image space, and thus, the inverse of $L_{X_{r-2:r-2}|\Xst}$ can be defined on range $L_{X_{r-2:r-2}|\Xst} \oplus \text{range} L_{X_{r-2:r-2}|\Xst}^{\perp}$, which is a dense subset of $\mathcal L^2(\mathcal A_l)$.

%Step 2: In order to show unique decomposition, we need to show that the operator $L_{X_{r-2:r-2}|\Xst}\mathcal{D}_{y_1, y_2 }L_{X_{r-2:r-2}|\Xst}^{-1}$, or $J_{y_1} J^{-1}_{y_2}$ is bounded. (I do not think $L_{X_{r-2:r-2}|\Xst}^{-1}$ is bounded. Thus I won't pursue this direction!)
%The main strategy is to show that its spectrum is a compact interval. I give a detailed proof below.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
